EIGEN: Event Influence GENeration using Pre-trained Language Models

Reasoning about events and tracking their influences is fundamental to understanding processes. In this paper, we present EIGEN - a method to leverage pre-trained language models to generate event influences conditioned on a context, nature of their influence, and the distance in a reasoning chain. We also derive a new dataset for research and evaluation of methods for event influence generation. EIGEN outperforms strong baselines both in terms of automated evaluation metrics (by 10 ROUGE points) and human judgments on closeness to reference and relevance of generations. Furthermore, we show that the event influences generated by EIGEN improve the performance on a "what-if" Question Answering (WIQA) benchmark (over 3% F1), especially for questions that require background knowledge and multi-hop reasoning.

==> sections/abstract.tex <==
\section*{Abstract}

% Understanding events and its influences is one of key aspects of commonsense knowledge understanding. In this paper, we propose a novel task of \textit{Dynamic Event Graph Generation}(DEGG), where our aim is to develop a framework for generating targeted event influence grounded in a context. Our framework uses a pre-trained language model and generates an \emph{influence graph} of an event based on the relationship and the hop in a reasoning chain. Our framework generates better influence graphs, compared to strong baselines both in terms of automated and human metrics. We also show that our generated influence can also improve downstream QA task, by simply augmenting it to an exisitng model. We improve performance on a recent procedural comprehension benchmark (WIQA) by about $\sim$3\% points in F1, particularly among questions that require reasoning with background knowledge.

% which takes the query event, a set of related questions and a paragraph of the context description as the input, and produces a graph of events (the nodes) and multi-type relations (the edges) on the fly as the output.  To address this challenge, we propose to adapt/extend the BERT's fine-tuning process to enable effective use of masked language modeling for contextualized node representation learning in the recursive process of graph induction conditioned on each input query and associated questions.  Evaluating our DEGG-induced graphs in
% comparison with human-annotated graphs in the WIQA benchmark dataset, we found DEGG outperforming other representative methods in event influence graph induction.  Additionally,  evaluating DEGG in reading comprehension (question asnwering) as a down-stream task on WIQA, we observed DEGG significantly outperforming other state-of-the-art QA methods. 

%  new challenging task, namely \textit{Dynamic Event Graph Generation} (DEGG), which takes the query event, a set of related questions and a paragraph of the context description as the input, and produces a graph of events (the nodes) and multi-type relations (the edges) on the fly as the output.  To address this challenge, we propose to adapt/extend the BERT's fine-tuning process to enable effective use of masked language modeling for contextualized node representation learning in the recursive process of graph induction conditioned on each input query and associated questions.  Evaluating our DEGG-induced graphs in
% comparison with human-annotated graphs in the WIQA benchmark dataset, we found DEGG outperforming other representative methods in event influence graph induction.  Additionally,  evaluating DEGG in reading comprehension (question asnwering) as a down-stream task on WIQA, we observed DEGG significantly outperforming other state-of-the-art QA methods.  

% \yy{Please check the accuracy of the above wording as I do not fully understand your method description (key part is still missing) and the evaluation results.  In other words, my abstract draft is based on guessing in certain degree. As a general commend, Title, Abstract and Introduction should be given before your share with advisors.  }

==> sections/introduction_v2_backup.tex <==
\section{Introduction}

\begin{figure*}[!t]
    {\includegraphics[width=\textwidth]{imgs/wiqa-gen-v11.pdf}}
    \caption{An overview of our methodology. The procedural text describes the process of \emph{photosynthesis}. For this example, we generate the influence graph for the event \emph{more sunlight}. The influence graph is generated for the relation types - \emph{helps, hurt by, helped by} and hops = $\{1,2\}$. A sample output influence graph shows the generated events - \emph{bright skies, cloudy skies, plants trap sunlight, and plants grow taller}} 
    \label{fig:intro-example}
\end{figure*}
\am{Things we want to talk about:
\begin{enumerate}
    \item What are event influences, and why are they important?
    \item What is the prior work, what is the gap?
    \item What are we doing in this work?
    \item Our contributions
\end{enumerate}
}

% Given a context and an event, humans can easily anticipate and reason about its causal influences: what is the effect of an event, what might cause an event to be less likely, and how different events influence each other in a process.\am{should we add ?}
% \sm{First sentence should reflect `what are event influences'. This first sentence seems redundant.}
% \ar{I agree. Define event influences and then you can retain the sentence with `humans are adept...'}
Humans are adept at anticipating and reasoning about events and their causal effects~(influences) on other events.
%However, performing such \textit{event influence reasoning} is extremely challenging for machines.
% An event influence describes its causal effects on other events for a process and understanding such event influences is fundamental to qualitative reasoning about processes.
%: what is the effect of an event, what might cause an event to be less likely, and how different events influence each other in a process.\am{should we add ?}
Consider these questions - \emph{Would it rain more if we plant more trees?},  \emph{What would help the water in boiling faster?} - answering these questions requires the ability to comprehend the complex processes of \emph{plant growth} and \emph{water boiling} and the capacity to reason about how various events influence each other in these processes that are typically implicit in text. Hence, reasoning about events and influences remains a significant challenge for machines.
% For instance, \emph{plant more trees} event positively influences \emph{more rain}. 
% For instance, \emph{plant more trees} event positively influences \emph{more rain}, and \emph{adding heat} will help  \emph{water in boiling faster}.

% \ar{I would even add concrete examples here of what could make water boil faster. Maybe we can refer to figure 1 and use it as a running example to explain ?}
% \sm{This is a different point than `what are event influences and an example'. So it should be a separate para. Its ok if they are short paras.}


Previous approaches have studied event understanding in the context of extraction \cite{chambers-jurafsky-2008-unsupervised,Yang2019ExploringPL,wang-etal-2019-open}, temporal reasoning~\cite{ning2018joint,vashishtha2019fine}, and entity tracking~\cite{dalvi-etal-2018-tracking}.
However, these systems are primarily \emph{extractive} --- they reason about events already mentioned in the text. This limits their ability to be integrated to downstream tasks that require implicit reasoning about events: such as question answering (\qa)~\cite{tandon2019wiqa}, reasoning about qualitative relationships~\cite{tafjord2019quarel}, and physical commonsense reasoning~\cite{sap2019atomic,bisk2020piqa}.
The task of \emph{generating event influences} in unseen contexts is still an open challenge. 
Two major hinder such exploration: i) lack of large-scale stand-alone datasets to study event influences, and ii) a formualtion of the event influence generation task that can be used in a generative setting/a framework for adapting language models for event influence generation
% Such an exploration entails two major challenges: i) lack of large-scale stand-alone datasets to study event influences, and ii) a framework for training models to generate event influences.
% a framework to generate event reasoning chains conditioned on the context and nature of the influence.
%primarily due to the lack of large-scale stand-alone datasets to study event influences.\am{Also add lack of a framework. Both the challenges should be added here}
% Such an exploration entails two major challenges: i) lack of large-scale stand-alone datasets to study event influences, and ii) a framework to leverage \plm to adapt them for event influence generation.
We bridge this gap \yyc{in this work}{} by first deriving a large corpus based on WIQA~\cite{tandon2019wiqa} dataset that can be used for the generation of event influences conditioned on context, relationship between the events, and the distance between them in a reasoning chain.
Next, we propose a framework--\ours, that takes a context and an event, and generates its influences both in forward and backward directions.
An example use of our framework is shown in Figure \ref{fig:intro-example}.
In the figure, nodes represent the event influences and the edges represent the nature of the influence (relation) between them. 
These relations can either be positive (when one event \textit{helps} the occurrence of another) or negative (when one event \textit{hurts} the occurrence of another). 
The distance between any given pair of nodes (in terms of number of edges traversed) is denoted by \emph{hop}.

We leverage pretrained language models (\plm) to train \ours since they have shown promising evidence from recent work to encode a wide-range of knowledge from their pretraining corpus \cite{Bosselut2019COMETCT,petroni2019language,davison-etal-2019-commonsense}
and successful adaptation in downstream tasks \cite{yang2020g,kumar2020data,Guan2020AKP}.  
%Motivated by these successes, we investigate whether we can adapt \plm for the novel task of \emph{event influence generation} and determine empirically whether the generated event influences lead to downstream performance gains.
%\ours fine-tunes a \plm to generate novel event influences for unseen contexts using masked language modeling.
We show empirically that our framework generates high quality influences for an event, both in terms of automated metrics (by $\sim$ 10 ROUGE) and human metrics --- fluency, relevance and proximity to the reference text. 
Together, the overall framework can be seamlessly integrated into any downstream task.
In one such instance, we show how the event influences generated from \ours can be easily augmented to a downstream \qa task and improve its performance without any need for modifying the underlying model architecture.
In summary, our contributions are:
\begin{enumerate}
    % \item  We define the problem of target event-influence reasoning as a task of graph generation conditioned on context;
     \item We propose the task of \emph{event influence generation} and derive a large-scale dataset for the same. 
  
    \item We propose \ours, a framework to generate targeted influence nodes for an event. Our experiments show that \ours outperforms strong baselines in both automated and human evaluation. 

    \item We also validate our approach by augmenting generated influences to a downstream \qa dataset, improving over the state of the art by 3\% in overall accuracy, and by 8\% on the subset of questions that require implicit event-influence reasoning \footnote{All code and data will be released upon acceptance.}.
\end{enumerate}
    

==> sections/introv1.tex <==
\section{Introduction}
\subsection{Old Introduction}

Previous approaches have studied event understanding in the context of event extraction \cite{chambers-jurafsky-2008-unsupervised,Yang2019ExploringPL,wang-etal-2019-open}, temporal event reasoning~\cite{ning2018joint,vashishtha2019fine}, and Question-Answering~\cite{tandon2019wiqa,dalvi-etal-2018-tracking}.
However, these systems are primarily \emph{extractive} --- they reason about events already mentioned in the text, limiting their ability to be integrated to downstream tasks that require implicit reasoning about events. 
The task of generating event influence in unseen contexts is still an open challenge. 

Meanwhile, promising evidence from recent work attests to the ability of pretrained language models (\plm) to encode a wide-range of knowledge from their pretraining corpus \cite{Bosselut2019COMETCT,petroni2019language,davison-etal-2019-commonsense}, enabling their successful adaptation in downstream tasks \cite{yang2020g,kumar2020data,Guan2020AKP}.  
Motivated by these successes, we investigate whether we can adapt \plm for the novel task of \emph{event influence generation} and determine empirically whether the generated event influences lead to downstream performance gains.
% \sm{I think i) should go in the para where you explicitly mention the gap. }
Such an exploration entails two major challenges: i) lack of large-scale stand-alone datasets to study event influences, and ii) a framework to leverage \plm to adapt them for event influence generation. %reasoning recursively/conditionally/XYZ.
% \ar{This is slightly suggestive of us contributing the dataset, when we repurpose Wiqa for this task. I agree this is a challenge, but maybe we could do some reordering to make it clear that our real contribution is figuring out how to make PLMs good at this.}
%\sm{This should be the beginning of your 3rd para. It is also your main work.}

In this work, we address these challenges by first deriving a large corpus based on WIQA~\cite{tandon2019wiqa} dataset that can be used for the generation of event influences conditioned on context, relationship between the events, and the distance between them in a reasoning chain.
%To overcome this, we derive a large corpus based on WIQA \cite{tandon2019wiqa} dataset that can be used for the generation of event influences conditioned on context, relation type, and hop information.
%Our work proposes a framework that leverages pretrained language models for event understanding to answer the question: \emph{how can we dynamically generate influences of an event conditioned on a given context?}. 
% Next, we propose \ours framework - that takes a context and a target event, and generates its influences both in forward and backward directions. 
Next, we propose our framework, \ours, that takes a context and an event, and generates its influences both in forward and backward directions.
An example use of our framework is shown in Figure \ref{fig:intro-example}.
In the figure, nodes represent the event influences and the edges represent the nature of the influence (relation) between them. 
These relations can either be positive (when one event \textit{helps} the occurrence of another) or negative (when one event \textit{hurts} the occurrence of another). 
The distance between any given pair of nodes (in terms of number of edges traversed) is denoted by \emph{hop}.


\ours fine-tunes a \plm to generate novel event influences for unseen contexts using masked language modeling.
We show empirically that our framework generates high quality influences for an event, both in terms of automated metrics (by $\sim$ 10 ROUGE) and human metrics --- fluency, relevance and proximity to the reference text. 
Together, the overall framework can be seamlessly integrated into any downstream task.
In one such instance, we show how the event influences generated from \ours can be easily augmented to a downstream \qa task and improve its performance without any need for modifying the underlying model architecture. 

% \am{
% Clarify that we perform three kinds of evaluations:
% 1) Node level (BLEU),
% 2) Human eval, and finally
% 3) Graph level (we don't have to call it graph level, but we need to clearly identify the evaluation mode) (QA)
% }
% \am{
% Find a good place to say: Our work is similar in spirit to \comet
% }

% \shrimai{
% \begin{itemize}
%     \item Para 1: Why we need causal graphs, causal reasoning, causal expressions. Applications of being able to generate such causal text
%     \item Para 2: How pre-trained models have proven to be successful in multitude of NLP tasks. Hence, we want to use them for our goal
%     \item Para 3: Narrow the focus of this paper. Write the question here. Can also write about narrowing the scope of task.
%     \item Para 4: What we show in our paper - that we are able to distill graphs, useful for QA. Primary controbution of the work
% \end{itemize}
% }
% \lasha{Rewrite suggestion: 
% Identifying events and their causal influences is an important component in language understanding (can replace with intelligence or any other term here). Tracing these causal effects is important for several NLP applications including Question Answering, process tracking \lasha{add other natural language understanding applications here, causality is important in lots of places. Also add citations. WiQa, Quarel and quartz can be some good starting points. WSC challenge.} \dheeraj{add citations}.  Consider these examples: \emph{Would it rain more if we plant more trees?},  \emph{Would the water boil faster if we add some salt?}, answering these questions requires a model to have the ability to comprehend the complex events of \emph{plant growth} and \emph{water boiling} and the capacity to reason about how these events are influenced by other factors. 
% }
% \dheeraj{we had deliberately avoided causal because Ed told us. When I explained the project to him, he seemed to think the we extract causal expressions but not causality exactly. The original WIQA paper also didn't q........................................................................................................................................uite claim any causality. thats why we resorted to "event influences" rather than causality}
% \lasha{Thanks for the explanation, Dheeraj. That makes total sense. Should we also modify the title in that case ?} YUP, it was meant to be a placeholder anyways
% \am{extend this work as a generation task for a wider applicability}
% \am{how we define the problem more formally nd evaluate and veluate the graphs qualitatively and quantitavely, dont try to avoid the word novel}
% \am{wiqa talks about QA}
% \am{one to many mapping, every two nodes in the graph form a qa pair}
% \am{output is the instantiated nodes}

% \am{for this valueable source , we can add some ninfo}

\begin{figure*}[!t]
    {\includegraphics[width=\textwidth]{imgs/wiqa-gen-v11.pdf}}
    \caption{An overview of our methodology. The procedural text describes the process of \emph{photosynthesis}. For this example, we generate the influence graph for the event \emph{more sunlight}. The influence graph is generated for the relation types - \emph{helps, hurt by, helped by} and hops $1$, and $2$. A sample output influence graph shows the generated events - \emph{bright skies, cloudy skies, plants trap sunlight, plants grow taller}} 
    \label{fig:intro-example}
\end{figure*}
% \am{Define event influences}
The ability to reason about events and their influences is a vital component in understanding processes.
% Consider these questions - \emph{Would it rain more if we plant more trees?},  \emph{Would the water boil faster if we add some salt?} - answering these question requires a model to have the ability to comprehend the complex events of \emph{plant growth} and \emph{water boiling} and the capacity to reason about other events that are influenced these events (event influences).
Consider these questions - \emph{Would it rain more if we plant more trees?},  \emph{Would the water boil faster if we add some salt?} - answering these question requires a model to have the ability to comprehend the complex events of \emph{plant growth} and \emph{water boiling} and the capacity to reason about the how \yyc{}{such events influencing each other}.
%(event influences).
Understanding such events and tracing their influence chains is essential for end tasks like question answering (\qa)~\cite{tandon2019wiqa}, process tracking~\cite{dalvi-etal-2018-tracking}, reasoning about qualitative relationships~\cite{tafjord2019quarel} and physical commonsense reasoning~\citep{sap2019atomic}. 
%\lasha{Can we cite more general purpose NLP tasks? I think NLI and maybe Winograd schema or physical commonsense reasoning tasks must require reasoning about event influences?}. \dheeraj{I dont see a direction connection except physcial common sense, how do you think otehr takss will benefit ?}
%In this paper, we address this challenge of automatically generating influences for a given event. 

% Recent research in understanding events and their influences on other events has been primarily studied under the Question-Answering paradigm~\cite{tandon2019wiqa,dalvi-etal-2018-tracking}, severely limiting their wide-spread applicability beyond the specified task.
%Recent research in understanding events and their influences on other events has primarily been modeled as Question-Answering~\cite{tandon2019wiqa,dalvi-etal-2018-tracking}. 
Recent research in understanding and reasoning about event  influences include the modeling of influences among event pairs  and using such relationship to improve question answering tasks, and the recent studies on using large-scale pre-trained language models to generate commonsense knowledge graphs
%on other events has primarily modeled the task as one of Question-Answering~
\cite{tandon2019wiqa,dalvi-etal-2018-tracking}.
%Consequently, their focus is on predicting the relationship between two events, rather than generating new events.
%Improving upon these works, we aim to model understanding event influences as a generation task for its wider applicability.
% Improving upon these works, we aim to model understanding event influences as a generation task for its wider applicability.
%\am{Maybe add why they are limited? None of these criticisms is precise, it will be shot down}
%Several recent approaches have been proposed for generating commonsense knowledge graphs from large scale pre-trained language models~\citep{Bosselut2019COMETCT,Guan2020AKP}. We build upon these works, and adapt these general purpose generation strategies to reason about event influences towards generation of targeted and contextually relevant event influences.
%Several recent approaches have been proposed for generating commonsense knowledge graphs from large scale pre-trained language models
~\citep{Bosselut2019COMETCT,Guan2020AKP}.
Although those work are highly inspirational, open questions remain for further research, including: 
\begin{itemize}
    \item How can we \textit{dynamically} generate event influence graphs conditioned on user-specified event of interest, the related context, the relevant influence types and the lengths of influence chains?  
    \item How can we evaluate the quality and usefulness of system-generated event influence graphs?  What kinds of benchmark dataset and evaluation metrics do we need?
\end{itemize}
This paper aims to address the above challenges with the following contributions:
\begin{enumerate}
    \item  We define the problem event-influence based reasoning as the task of graph generation conditioned on context and other input information;
    \item We propose a novel approach, namely \ours, to induce the targeted influence graphs;
    \item We generate a new dataset for direct evaluation of system-induced event influence graphs;
    \item Our evaluation show the advantageous performance of \ours over strong baselines in both automated metrics and human evaluation.
\end{enumerate}
 
\yy{Aman: I stop here: you decide what you want to do with the rest of the introduction: you may delete them or more some to other sections.}

%We adapt these general purpose generation strategies for targeted and contextually relevant event influence generation.
%We believe that a study of event influences in a more general setting of generation would h a more generic generation
%\am{Instead of criticizing the work, you can say that we take inspiration from this work and we seek to do in-depth study of a specific problem event influence generation. How this influence graph generation process, }
%To this end, we propose adapting large-scale pre-trained language towards generating fine-grained \emph{contextualized event influence graphs} that can be easily integrated into any downstream task. 
% We define this task \emph{Dynamic Event Graph Generation}.

% \yy{"Inspired by the above work, this paper aims to further improve the current technologies for graph-based reasoning about the influences among events.  Specifically, we a novel framework for incorporating large scale pre-trained language models in the process of automated and dynamic generation of \textit{Contextualized Event Influence Graphs}.}
%This paper aims to address the challenge of generating event influence graphs as a generation task grounded in the context. <- this was the line, I've commented it out now
This paper aims to address the challenge of generating event influence graphs grounded in context.
An influence graph~\citep{tandon2019wiqa} describes how an event positively or negatively influences other events in a context. 
%We particularly focus on events that are present as nodes in an influence graph~\citep{tandon2019wiqa}, wherein each node  describes how an event positively or negatively influences other events in a context.
For a given context and an event, we generate its corresponding influences conditioned on a specified \emph{relation type} and the \emph{hop} information.
A relation type captures the nature of influence between the two events\footnote{does one event help or hurt the likelihood of the other} and the hop information captures the distance between the events in the reasoning chain.
%We propose a methodology to extract such human-curated influence graphs, we traverse 
%Using human-curated event influence graphs, we first create a dataset create  by tr
To this end, we propose \ours~- a novel method to fine-tune pre-trained language models for generating event influences based on a set of specified relation types and hops, allowing us to iteratively build an influence graph. %for the event which we denote by \ours. 
%To this end, we propose \ours~- a method that can leverage large pre-trained language models for the task.
%\ours can generate event influences based on a set of specified relation types and hops, allowing us to iteratively build event influence graphs~\citep{tandon2019wiqa}.
%generate event influences based on a set of specified relation types and hops, allowing us to iteratively build an influence graph.
Figure \ref{fig:intro-example} shows a sample influence graph generated for the event \emph{more sunlight} in the context of \emph{photosynthesis}. 

Our experiments show that \ours generates better influence graphs compared to strong baselines as measured by standard automatic generation metrics. 
We also show that outputs from \ours are more fluent, relevant, and closer to reference compared to other generation baselines.
% Furthermore, we evaluate the utility of the generated event influence graphs by augmenting the graph information in a downstream QA task \citep{tandon2019wiqa}.
Further, we demonstrate the utility of the generated event influence graphs, by utilizing them in a downstream \qa task~\citep{tandon2019wiqa}, finding that doing so improves over the current state-of-the-art \cite{tandon2019wiqa}. Specifically, we show gains for questions which require background knowledge and reasoning over longer hops. 
% Our results show that \ours improves over the current state-of-the-art for the task \cite{tandon2019wiqa}.
%by simply augmenting the event influence graphs, without modifying the underlying model architecture. 


%We also perform an empirical study to assess the quality of the generated events. The results indicate that our methodology performs better than baselines such as comet and an rnn based sequence to sequence models. We also provide an ablation over the two attributes of relation and hop to better understand the effect of our generations across multiple relations and hops. Furthermore, we evaluate the utility of the generated influence graphs by using them in downstream QA task. We find that ... (You can combine the previous para and talk about it here itself.

% \sm{Our primary contribution is casting the task of studying event influences as a generation task which is grounded in context/procedural text to restrict the scope of the events. Additional we demonstrate that pre-trained language models can be leveraged to generate these. We perform an empirical study to assess the quality of the generated events. The results indicate that our methodology performs better than baselines such as comet and an rnn based sequence to sequence models. We also provide an ablation over the two attributes of relation and hop to better understand the effect of our generations across multiple relations and hops. Furthermore, we evaluate the utility of the generated influence graphs by using them in downstream QA task. We find that ... (You can combine the previous para and talk about it here itself.) }

% \yy{introduce Figure 1 here, for describing the task with a concrete example.  And then, make clear statements about how this task or the problem settings are fundamentally different from previous work in graph-based commonsense reasoning about events. Then, you should discuss how the induced graphs should be evaluated: by human evaluation and by task-oriented evaluation (e.g., in QA).  After all the above, your are ready to summarize your main contributions in this paper. All the current paragraphs below should be either deleted or subsumed in this way of writing.}

% \notes{Who else has investigated this question? What are their approaches?} \notes{Have you introduced this task?} \notes{Better start from commonsense reasoning from the graph?}

To summarize, our contributions are: 
(1) We pose the problem of studying event influences as a generation task grounded in context,
(2) We propose \ours - a novel method that produces targeted event influences.
Our experiments show that \ours outperforms the 
%generated influence graphs are better than ones generated by 
baselines both in terms of automated generation metrics and human evaluation. We also show a comprehensive ablation study and analysis of the generated influences,
(3) Besides automated and human evaluation of generation quality, we validate our approach by observing improvements in a downstream \textsc{qa} task wherein we augment our generated influence graphs to the original dataset. 
We perform particularly well in questions that require background knowledge and multihop reasoning.\footnote{All code and data will be released upon acceptance.}
%(3) \am{rephrase} We also show a real-world use-case to validate our approach, where we augment the event influence graph to a downstream QA task. We improve the performance of best model of the QA task by simply augmenting our influence graphs and perform better particularly in questions that require background knowledge.\footnote{All the code and data will be released upon acceptance.}


% Pre-trained language models like \textsc{bert}, \textsc{xlnet}, and \textsc{gpt2} have received a lot of attention recently for establishing state of the art on an array of natural language understanding tasks. These models are typically trained on gigabytes of text scraped from the internet and have billions of parameters. For instance, gpt2 has 1.35 billion parameters and was trained on 40 \textsc{gb} of text. While much work has been done on finding out how much knowledge do these large scale language models contain\am{add citations on LM kb work}, it's not entirely clear if they can be tweaked to learn more complicated properties of language. 

% In this work, we focus on the following question: Can language models be trained to learn about \emph{what-if} changes? That is, given a process, can we reason about the varied outcomes that would result from varying the steps or the inputs of the process? For instance, would it rain more if we plant more trees? Would the water boil faster if we add some salt?
%\am{the following paragraph has already been added to section 2.1, feel free to uncomment/move etc.}
%As stated, the question we pose is too grandiose to be tackled in a single study. Most of the systems are sensitive to changes. Further, the types of changes are large, varied, and depend on more than one input variable. Fortunately, \citet{tandon2019wiqa} released a dataset, \textsc{wiqa}, that circumscribes the scope of our question without diluting it in importance or spirit. The dataset consists of 2107 influence graphs over 300 scientific processes like the digestion of food and photosynthesis. The influence graph for a process consists of nodes that capture events or states pertaining to the process, and two kinds of edges: \emph{helps} or \emph{hurts} for one system state/event helping or hurting the realization of the other. Focusing on this dataset allows us to limit the scope of our work to two kinds of what-if changes (helping or hurting) on a set of reasonably structured processes. While this may appear to be superficially limiting, the demarcation of scope is conducive to an exhaustive analysis, and we believe that furthers the current understanding of language models and their capabilities. Finally, we'd like to note that our exploration addresses a subset of causality, but is orthogonal to the existing work as they address causality of outcome independent of the context. 
